Multiplayer Reach-Avoid Games via Pairwise Outcomes

A multiplayer reach-avoid game is a differential game between an attacking team with NA attackers and a defending team with ND defenders playing on a compact domain with obstacles. The attacking team aims to send M of the NA attackers to some target location, while the defending team aims to prevent that by capturing attackers or indefinitely delaying attackers from reaching the target. Although the analysis of this game plays an important role in many applications, the optimal solution to this game is computationally intractable when NA>1 or ND>1. In this paper, we present two approaches for the NA=ND=1 case to determine pairwise outcomes, and a graph theoretic maximum matching approach to merge these pairwise outcomes for an NA,ND>1 solution that provides guarantees on the performance of the defending team. We will show that the four-dimensional Hamilton-Jacobi-Isaacs approach allows for real-time updates to the maximum matching, and that the two-dimensional "path defense" approach is considerably more scalable with the number of players while maintaining defender performance guarantees.

==> comparison.tex <==
% !TEX root = multiplayer_reach_avoid_games.tex
\section{Comparison Between the HJI and Path Defense Approaches}
\label{sec:comparison}
The HJI approach holds an advantage over the path defense approach in terms of optimality. The HJI solution to the two-player reach-avoid game computes the entire 4D reach-avoid set and gives the optimal closed-loop control strategies for each attacker-defender pair; on the other hand, the path defense solution computes 2D slices of the 4D reach-avoid set sliced at the attacker position, and provides a more conservative semi-open-loop control strategy to the defenders. As a result, the defender winning regions computed in the path defense approach tend to be smaller than those computed in the HJI approach, as seen in Figures \ref{fig:comp_ol} and \ref{fig:comp_ml}. The degree of conservatism is more pronounced when the attacker is slower than the defender and when the domain contains large obstacles, as seen in Figure \ref{fig:comp_ml}. Furthermore, because the HJI approach computes entire 4D reach-avoid sets, very little additional computation overhead is required for updating pairwise outcomes as the players move during the course of the game.

The path defense approach trades off optimality for computation complexity for the case where $\velai{i}\le \velbi{j} \; \forall i,j$. Because the HJI approach involves solving an HJI PDE in a 4D space, the computation time tends to be long and the memory requirements are high. Typically, a single 4D HJI PDE takes approximately half an hour to solve on a relative coarse grid in each dimension. Computation of a 2D slice using the path defense approach can be done on much finer grids with the same amount of memory, and takes only a few seconds. Furthermore, when computing all pair-wise outcomes, the number of 2D slice computations required in path defense approach only scales with $\N$, the number of attackers, whereas the number of 4D HJI PDEs that needs to be solved is $\N^2$.

